Deep Audio-Visual Singing Voice Transcription based on Self-Supervised Learning Models

Singing voice transcription converts recorded singing audio to musical notation. Sound contamination (such as accompaniment) and lack of annotated data make singing voice transcription an extremely difficult task. We take two approaches to tackle the above challenges: 1) introducing multimodal learning for singing voice transcription together with a new multimodal singing dataset, N20EMv2, enhancing noise robustness by utilizing video information (lip movements to predict the onset/offset of notes), and 2) adapting self-supervised learning models from the speech domain to the singing voice transcription task, significantly reducing annotated data requirements while preserving pretrained features. We build a self-supervised learning based audio-only singing voice transcription system, which not only outperforms current state-of-the-art technologies as a strong baseline, but also generalizes well to out-of-domain singing data. We then develop a self-supervised learning based video-only singing voice transcription system that detects note onsets and offsets with an accuracy of about 80\%. Finally, based on the powerful acoustic and visual representations extracted by the above two systems as well as the feature fusion design, we create an audio-visual singing voice transcription system that improves the noise robustness significantly under different acoustic environments compared to the audio-only systems.

==> tables/criterion_cmp.tex <==
\begin{table}
\caption{Comparison of labeling criteria between ISMIR2014 and MIR-ST500 datasets.}
	\centering
	\begin{tabular}{l|c|c}
		\toprule
		  Dataset & \textbf{ISMIR2014} & \textbf{MIR-ST500} \\
		\midrule
		Onset & \makecell[l]{At the beginning of voiced \\ segments, excluding unvoiced \\  segments and voiced consonants \\ such as ’l’, ’m’, ’n’} & \makecell[l]{At any place within the \\ leading unvoiced segment \\ before the voiced segment} \\
        \midrule
        Offset & No clear guidance & \makecell[l]{At the time annotators \\ think the voice ends} \\
        \midrule
        Pitch & Cents & Semitone \\
		\bottomrule
	\end{tabular}
    \label{tbl-criterion_cmp}
\end{table}

==> tables/exp_B1.tex <==


\begin{table}[t]
\caption{COnPOff / COnP / COn F1-score (\%) of baseline and our A-SVT system on MIR-ST500 test set / TONAS / ISMIR2014. Both SVT systems are trained on the MIR-ST500 train set.}
	\centering
	\begin{tabular}{l|l|c|c}
		\toprule
		Dataset & Metric (\%) $\uparrow$ & Baseline \cite{wang2021preparation} & Ours \\
		\midrule
		\multirow{3}{6em}{\textbf{MIR-ST500}} & COnPOff &  45.78 & \textbf{52.39} (\textbf{{\color{teal}+\,\,\,6.61}}) \\
		& COnP & 66.63 & \textbf{70.73} (\textbf{{\color{teal}+\,\,\,4.10}}) \\
		& COn & 75.44 & \textbf{78.32} (\textbf{{\color{teal}+\,\,\,2.88}}) \\
		\midrule
		\multirow{3}{6em}{\textbf{TONAS}} & COnPOff & \,\,9.57  & \textbf{12.71} (\textbf{{\color{teal}+\,\,\,3.14}}) \\
		& COnP & 19.65  & \textbf{25.24} (\textbf{{\color{teal}+\,\,\,5.59}}) \\
		& COn & 42.41  & \textbf{52.77} (\textbf{{\color{teal}+10.36}}) \\
		\midrule
		\multirow{3}{6em}{\textbf{ISMIR2014}} & COnPOff &  49.55  & \textbf{52.36} (\textbf{{\color{teal}+\,\,\,2.81}}) \\
		& COnP & 63.63  & \textbf{70.38} (\textbf{{\color{teal}+\,\,\,6.75}}) \\
		& COn & 79.16  & \textbf{92.77} (\textbf{{\color{teal}+13.61}}) \\
		\bottomrule
	\end{tabular}
    
    \label{tbl-exp-B1}
\end{table}
